Generalized Veneziano and Virasoro amplitudes

We analyze so-called generalized Veneziano and generalized Virasoro amplitudes. Under some physical assumptions, we find that their spectra must satisfy an over-determined set of non-linear recursion relations. The recursion relation for the generalized Veneziano amplitudes can be solved analytically and yields a two-parameter family which includes the Veneziano amplitude, the one-parameter family of Coon amplitudes, and a larger two-parameter family of amplitudes with an infinite tower of spins at each mass level. In the generalized Virasoro case, the only consistent solution is the string spectrum.

==> 2023_02_23_Geiser, Lindwasser_GenVenVir_v3/figure1.tex <==
\begin{figure}

\centering

\begin{tikzpicture}

\begin{axis}
[
    width = 1\textwidth,
    height = 0.7\textwidth,
    xmin = 0, xmax = 1.5,
    ymin = 0, ymax = 1.5,
    xtick = {0,1},
    ytick = {1},
    extra y ticks = {0},
    extra y tick labels = \empty,
    xlabel = {$x$},
    ylabel = {$y$},
    x label style = {at={(current axis.right of origin)}, anchor=west},
    y label style = {at={(current axis.north west)}, rotate=-90, anchor=south},
    axis lines = left,
    legend cell align = {left},
    legend pos = north west,
    legend entries =
    {
        % \, string spectrum ($x=y=1$)$\vphantom{\tfrac{(}{(}}$,
        % \, \makebox[\widthof{string spectrum}][l]{Coon spectra} ($y=x^2$)$\vphantom{\tfrac{(}{(}}$,
        % \, \makebox[\widthof{string spectrum}][l]{$r$-type spectra} ($y=\frac{x(1+x)}{(3-x)}$),
        % \, $p$-type spectra$\vphantom{\tfrac{(}{(}}$,
        % \, unphysical spectra$\vphantom{\tfrac{(}{(}}$
        \, string spectrum $x=y=1$,
        \, \makebox[\widthof{string spectrum}][l]{Coon spectra} \smash{$y=x^2$},
        \, \makebox[\widthof{string spectrum}][l]{$r$-type spectra} \smash{$y=x(1+x)/(3-x)$},
        \, $p$-type spectra,
        \, unphysical spectra
    }
]

\addlegendimage{only marks, mark size = 2pt, fill = green}
\addlegendimage{ultra thick, color = black}    
\addlegendimage{ultra thick, color = black, densely dashed}
\addlegendimage{only marks, mark = square*, mark size = 4pt, color = yellow!40}
\addlegendimage{only marks, mark = square*, mark size = 4pt, color = red!30}

\path[name path = xtop] (0,1.5) -- (1.5,1.5);
\path[name path = xbottom] (0,0) -- (1.5,0);

\addplot
[
    name path = c,
    domain = 0:1.5, 
    ultra thick,
	black,
    smooth
]
{x*x};

\addplot
[
    name path = r,
    domain = 0:1, 
    ultra thick,
	black,
    densely dashed,
    smooth
]
{x*(1+x)/(3-x)};
  
\addplot
[
    only marks,
    mark size = 4pt,
    fill = green
]
coordinates {(1,1)};

\addplot[yellow!40]
fill between
[
    of = r and c,
    soft clip = {domain = 0:1},
    on layer = axis background
];

\addplot[yellow!40]
fill between
[
    of = c and xbottom,
    soft clip = {domain = 0:1.2247},
    on layer = axis background
];

\addplot[yellow!40]
fill between
[
    of = xtop and xbottom,
    soft clip = {domain = 1.224:1.5},
    on layer = axis background
];

\addplot[red!30]
fill between
[
    of = r and xtop,
    soft clip = {domain = 0:1},
    on layer = axis background
];

\addplot[red!30]
fill between
[
    of = c and xtop,
    soft clip = {domain = 0.99:1.2247},
    on layer = axis background
];

\end{axis}

\end{tikzpicture}

\caption{The two-parameter space of solutions to the generalized Veneziano amplitude constraints. The point ${x=y=1}$ corresponds to the string spectrum. The solid black line corresponds to the one-parameter subspace of Coon spectra. The dashed black line corresponds to the one-parameter subspace of $r$\nobreakdash-type spectra. The yellow region corresponds to the two-parameter subspace of $p$\nobreakdash-type spectra. The red region corresponds to unphysical spectra with negative mass squared.}

\label{fig:Ven1}

\end{figure}

==> 2023_02_23_Geiser, Lindwasser_GenVenVir_v3/figure2.tex <==
\begin{figure}

\centering

\begin{tikzpicture}

\begin{axis}
[
    width = 1\textwidth,
    height = 0.7\textwidth,
    xmin = 0, xmax = 1.5,
    ymin = 0, ymax = 1.5,
    xtick = {0,2/3,1},
    ytick = {1},
    extra y ticks = {0},
    extra y tick labels = \empty,
    xticklabels = {$0$, $\tfrac{2}{3}$, $1$},
    xlabel = {$x$},
    ylabel = {$y$},
    x label style = {at={(current axis.right of origin)}, anchor=west},
    y label style = {at={(current axis.north west)}, rotate=-90, anchor=south},
    axis lines = left,
    legend cell align = {left},
    legend pos = north west,
    legend entries =
    {
        \, string spectrum,
        \, Coon spectra,
        \, $r$-type spectra,
        \, unitary in $d \leq 4$,
        \, unitary in $d \leq 6$,
        \, unitary in $d \leq 10$,
        \, unitary in all $d$,
        \, non-unitary,
        \, unphysical spectra
    }
]

\path[name path = xtop] (0,1.5) -- (1.5,1.5);
\path[name path = xbottom] (0,0) -- (1.5,0);

\addlegendimage{only marks, mark size = 2pt, fill = green}
\addlegendimage{ultra thick, color = black}    
\addlegendimage{ultra thick, color = black, densely dashed}
\addlegendimage
{
    only marks,
    mark = square*,
    color = green!40!white,
    mark size = 4pt
}   

\addlegendimage
{
    only marks,
    mark = square*,
    color = green!80!black,
    mark size = 4pt
}    

\addlegendimage
{
    only marks,
    mark = square*,
    color = green!45!black,
    mark size = 4pt
}

\addlegendimage
{
    only marks,
    mark = square*,
    color = blue!60,
    mark size = 4pt
}

\addlegendimage
{
    only marks,
    mark = square*,
    color = yellow!40,
    mark size = 4pt
}

\addlegendimage
{
    only marks,
    mark = square*,
    color = red!30,
    mark size = 4pt
}

\addplot
[
    name path = c,
    domain = 0:1.5, 
]
{x*x};

\addplot
[
    domain = 0.666:1.5, 
    ultra thick,
	black,
    smooth,
    opacity = 0.75
]
{x*x};

\addplot
[
    domain = 0:0.667, 
    ultra thick,
	blue!60,
    smooth,
]
{x*x};

\addplot
[
    name path = r,
    domain = 0:1, 
    ultra thick,
	black,
    densely dashed,
    smooth,
    opacity = 0.75
]
{x*(1+x)/(3-x)};

\addplot
[
    only marks,
    mark size = 3pt,
    fill = green
]
coordinates {(1,1)};

\addplot
[
    name path = d4,
    smooth,
    green!40!white,
    on layer = axis background
]
file[skip first]{d4unitary.dat};

\addplot
[
    name path = d6,
    smooth,
    green!80!black,
    on layer = axis background
]
file[skip first]{d6unitary.dat};

\addplot
[
    name path = d10,
    smooth,
    green!45!black,
    on layer = axis background
]
file[skip first]{d10unitary.dat};

\addplot
[
    samples = 500,
    name path = fm1,
    domain = 0:0.667,
    on layer = axis background,
	blue!60,
    smooth,
]
{ x*x*(6+x-3*x*x-sqrt(9-6*x-11*x*x))/(9-3*x-5*x*x+3*x*x*x) };

\addplot
[
    samples = 200,
    name path = fm2,
    domain = 0.666:0.672,
    on layer = axis background,
	blue!60,
    smooth,
]
{ x*x*(6+x-3*x*x-sqrt(9-6*x-11*x*x))/(9-3*x-5*x*x+3*x*x*x) };

\addplot
[
    samples = 200,
    name path = fp,
    domain = 0.666:0.672,
    on layer = axis background,
	blue!60,
    smooth,
]
{ x*x*(6+x-3*x*x+sqrt(9-6*x-11*x*x))/(9-3*x-5*x*x+3*x*x*x) };

\addplot
[
    name path = f0,
    domain = 0:0.667, 
    on layer = axis background,
	blue!60,
    smooth,
]
{ x*x };

\addplot[yellow!40]
fill between
[
    of = r and c,
    soft clip = {domain = 0:1},
    on layer = axis background
];

\addplot[yellow!40]
fill between
[
    of = c and xbottom,
    soft clip = {domain = 0:1.2247},
    on layer = axis background
];

\addplot[yellow!40]
fill between
[
    of = xtop and xbottom,
    soft clip = {domain = 1.224:1.5},
    on layer = axis background
];
 
\addplot[green!40!white] fill between [of=r and d4, on layer = axis background];
\addplot[green!80!black] fill between [of=r and d6, on layer = axis background];
\addplot[green!45!black] fill between [of=r and d10, on layer = axis background];

\addplot[blue!60] fill between [of=fm1 and f0, on layer = axis background];
\addplot[blue!60] fill between [of=fm2 and fp, on layer = axis background];

\addplot[red!30]
fill between
[
    of = r and xtop,
    soft clip = {domain = 0:1},
    on layer = axis background
];

\addplot[red!30]
fill between
[
    of = c and xtop,
    soft clip = {domain = 0.99:1.2247},
    on layer = axis background
];

\end{axis}

\end{tikzpicture}

\caption{The two-parameter space of solutions to the generalized Veneziano amplitude constraints with unitary regions in various dimensions. The blue region is unitary in all dimensions and includes the Coon amplitudes with ${0 < q \leq \frac{2}{3}}$. The dark green region is unitary in ${d \leq 10}$ and includes the Veneziano amplitude at ${x=y=1}$. The middle green region is unitary in ${d \leq 6}$. The light green region is unitary in ${d \leq 4}$. The blue region was computed analytically, and the green regions were computed by numerically analyzing the first few partial wave coefficients $c_{n,j}$.}

\label{fig:Ven2}

\end{figure}

==> 2023_02_23_Geiser, Lindwasser_GenVenVir_v3/preambledefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Nick Geiser
% ngeiser@physics.ucla.edu
% last updated 2022/08/02
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase calligraphic shorthand via \mathcal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase bold shorthand via \boldsymbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bfA}{\boldsymbol{A}}
\newcommand{\bfB}{\boldsymbol{B}}
\newcommand{\bfC}{\boldsymbol{C}}
\newcommand{\bfD}{\boldsymbol{D}}
\newcommand{\bfE}{\boldsymbol{E}}
\newcommand{\bfF}{\boldsymbol{F}}
\newcommand{\bfG}{\boldsymbol{G}}
\newcommand{\bfH}{\boldsymbol{H}}
\newcommand{\bfI}{\boldsymbol{I}}
\newcommand{\bfJ}{\boldsymbol{J}}
\newcommand{\bfK}{\boldsymbol{K}}
\newcommand{\bfL}{\boldsymbol{L}}
\newcommand{\bfM}{\boldsymbol{M}}
\newcommand{\bfN}{\boldsymbol{N}}
\newcommand{\bfO}{\boldsymbol{O}}
\newcommand{\bfP}{\boldsymbol{P}}
\newcommand{\bfQ}{\boldsymbol{Q}}
\newcommand{\bfR}{\boldsymbol{R}}
\newcommand{\bfS}{\boldsymbol{S}}
\newcommand{\bfT}{\boldsymbol{T}}
\newcommand{\bfU}{\boldsymbol{U}}
\newcommand{\bfV}{\boldsymbol{V}}
\newcommand{\bfW}{\boldsymbol{W}}
\newcommand{\bfX}{\boldsymbol{X}}
\newcommand{\bfY}{\boldsymbol{Y}}
\newcommand{\bfZ}{\boldsymbol{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase bold shorthand via \boldsymbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bfa}{\boldsymbol{a}}
\newcommand{\bfb}{\boldsymbol{b}}
\newcommand{\bfc}{\boldsymbol{c}}
\newcommand{\bfd}{\boldsymbol{d}}
\newcommand{\bfe}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bfg}{\boldsymbol{g}}
\newcommand{\bfh}{\boldsymbol{h}}
\newcommand{\bfi}{\boldsymbol{i}}
\newcommand{\bfj}{\boldsymbol{j}}
\newcommand{\bfk}{\boldsymbol{k}}
\newcommand{\bfl}{\boldsymbol{l}}
\newcommand{\bfm}{\boldsymbol{m}}
\newcommand{\bfn}{\boldsymbol{n}}
\newcommand{\bfo}{\boldsymbol{o}}
\newcommand{\bfp}{\boldsymbol{p}}
\newcommand{\bfq}{\boldsymbol{q}}
\newcommand{\bfr}{\boldsymbol{r}}
\newcommand{\bfs}{\boldsymbol{s}}
\newcommand{\bft}{\boldsymbol{t}}
\newcommand{\bfu}{\boldsymbol{u}}
\newcommand{\bfv}{\boldsymbol{v}}
\newcommand{\bfw}{\boldsymbol{w}}
\newcommand{\bfx}{\boldsymbol{x}}
\newcommand{\bfy}{\boldsymbol{y}}
\newcommand{\bfz}{\boldsymbol{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase Fraktur shorthand via \mathfrak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mfA}{\mathfrak{A}}
\newcommand{\mfB}{\mathfrak{B}}
\newcommand{\mfC}{\mathfrak{C}}
\newcommand{\mfD}{\mathfrak{D}}
\newcommand{\mfE}{\mathfrak{E}}
\newcommand{\mfF}{\mathfrak{F}}
\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfH}{\mathfrak{H}}
\newcommand{\mfI}{\mathfrak{I}}
\newcommand{\mfJ}{\mathfrak{J}}
\newcommand{\mfK}{\mathfrak{K}}
\newcommand{\mfL}{\mathfrak{L}}
\newcommand{\mfM}{\mathfrak{M}}
\newcommand{\mfN}{\mathfrak{N}}
\newcommand{\mfO}{\mathfrak{O}}
\newcommand{\mfP}{\mathfrak{P}}
\newcommand{\mfQ}{\mathfrak{Q}}
\newcommand{\mfR}{\mathfrak{R}}
\newcommand{\mfS}{\mathfrak{S}}
\newcommand{\mfT}{\mathfrak{T}}
\newcommand{\mfU}{\mathfrak{U}}
\newcommand{\mfV}{\mathfrak{V}}
\newcommand{\mfW}{\mathfrak{W}}
\newcommand{\mfX}{\mathfrak{X}}
\newcommand{\mfY}{\mathfrak{Y}}
\newcommand{\mfZ}{\mathfrak{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase Fraktur shorthand via \mathfrak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase blackboard bold (doublestroke) shorthand via \mathbb
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase Greek shorthand
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\ve}{\varepsilon}
% \zeta
% \eta
\renewcommand{\th}{\theta}
\newcommand{\vth}{\vartheta}
% \iota
\newcommand{\kap}{\kappa}
\newcommand{\vkap}{\varkappa}
\newcommand{\lam}{\lambda}
% \mu
% \nu
% \xi
% \omicron = o
% \pi
\newcommand{\vpi}{\varpi}
% \rho
\newcommand{\vrho}{\varrho}
\newcommand{\sig}{\sigma}
\newcommand{\vsig}{\varsigma}
% \tau
\newcommand{\ups}{\upsilon}
\newcommand{\f}{\varphi}
\newcommand{\vf}{\varphi}
% \chi
% \psi
\newcommand{\om}{\omega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase Greek shorthand
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Alpha = A
% \Beta = B
\newcommand{\G}{\Gamma}
\newcommand{\vG}{\varGamma}
\newcommand{\D}{\Delta}
\newcommand{\vD}{\varDelta}
% \Epsilon = E
% \Zeta = Z
% \Eta = H
\newcommand{\Th}{\Theta}
\newcommand{\vTh}{\varTheta}
% \Iota = I
% \Kappa = K
\newcommand{\Lam}{\Lambda}
\newcommand{\vLam}{\varLambda}
% \Mu = M
% \Nu = N
% \Xi
\newcommand{\vXi}{\varXi}
% Omicron = O
% \Pi
\newcommand{\vPi}{\varPi} 
% \Rho = P
\newcommand{\Sig}{\Sigma}
\newcommand{\vSig}{\varSigma}
% \Tau = T
\newcommand{\Ups}{\Upsilon}
\newcommand{\vUps}{\varUpsilon} 
\newcommand{\F}{\Phi} 
\newcommand{\vF}{\varPhi} 
% \Chi = X
% \Psi
\newcommand{\vPsi}{\varPsi}
\newcommand{\Om}{\Omega}
\newcommand{\vOm}{\varOmega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% delimiter shorthand
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\p}{\partial}

% 3-argument "thermodynamics" partial derivative
\newcommand{\dthermo}[3]{\left( \frac{\partial #1}{\partial #2} \right)_{#3}}

% math operators
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator*{\Res}{Res}

% better real and imaginary parts
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

% floor and ceiling
\newcommand{\floor}[1]{\cramped{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{\cramped{\left\lceil #1 \right\rceil}}

% extendable tilde for asymptotic expressions
\newcommand{\widesim}[2][1.5]{
  \mathrel{\overset{#2}{\scalebox{#1}[1]{$\sim$}}}
}

% small text-style symbols
\newcommand{\tsum}{\textstyle\sum\nolimits}
\newcommand{\tprod}{\textstyle\prod\limits}
\newcommand{\half}{\tfrac{1}{2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% negative phantom space
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\negphantom}[1]{
    \ifmmode\settowidth{\dimen0}{$#1$}
    \else\settowidth{\dimen0}{#1}
    \fi
    \hspace*{-\dimen0}}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mask: center in box with specified width
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Note to self: rewrite this function using \makebox and \settowidth
\makeatletter
\newcommand{\mask}[2]{{\mathpalette\mask@{{#1}{#2}}}}
\newcommand{\mask@}[2]{\mask@@{#1}#2}
\newcommand{\mask@@}[3]{%
  \settowidth{\dimen@}{$\m@th#1#2$}%
  \makebox[\dimen@]{$\m@th#1#3$}%
}
\makeatother
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Eric D'Hoker's formatting defs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sm}{\smallskip}
\newcommand{\no}{\nonumber}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% future typesetting projects
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Condense the definitions at top of this document using for-loop.
% Figure out consistent delimiter spacing with \left and \right. I think these commands add some unnecessary white space.
% Find way to consistently reduce space between +, -, etc. in long equations.
% Find way to uniformize vertical spacing in multiline equations.
% Why do the \floor, \ceil, \bmatrix brackets look bigger in JHEP published version of my 2021 paper?


